Green-Schwarz superstring on the lattice

We consider possible discretizations for a gauge-fixed Green-Schwarz action of Type IIB superstring. We use them for measuring the action, from which we extract the cusp anomalous dimension of planar $\mathcal{N}=4$ SYM as derived from AdS/CFT, as well as the mass of the two $AdS$ excitations transverse to the relevant null cusp classical string solution. We perform lattice simulations employing a Rational Hybrid Monte Carlo (RHMC) algorithm and two Wilson-like fermion discretizations, one of which preserves the global $SO(6)$ symmetry of the model. We compare our results with the expected behavior at various values of $g=\frac{\sqrt{\lambda}}{4\pi}$. For both the observables, we find a good agreement for large $g$, which is the perturbative regime of the sigma-model. For smaller values of $g$, the expectation value of the action exhibits a deviation compatible with the presence of quadratic divergences. After their non-perturbative subtraction the continuum limit can be taken, and suggests a qualitative agreement with the non-perturbative expectation from AdS/CFT. Furthermore, we detect a phase in the fermion determinant, whose origin we explain, that for very small $g$ leads to a sign problem not treatable via standard reweigthing. The continuum extrapolations of the observables in the two different discretizations agree within errors, which is strongly suggesting that they lead to the same continuum limit. Part of the results discussed here were presented earlier in arXiv:1601.04670.

==> so6/run_table.tex <==
\begin{tabular}{ccccccc}
\toprule
$g$ & $T/a\times L/a$ & $Lm$ & $am$ & $\tau_{\rm int}^{S}$ & $\tau_{\rm int}^{m_x}$ & statistic [MDU] \\
\midrule
  5 & $16 \times   8$ &  4  & 0.50000 & 0.8 & 2.2 & 900 \\
    & $20 \times  10$ &  4  & 0.40000 & 0.9 & 2.6 & 900 \\
    & $24 \times  12$ &  4  & 0.33333 & 0.7 & 4.6 & 900,1000 \\
    & $32 \times  16$ &  4  & 0.25000 & 0.7 & 4.4 & 850,1000 \\
    & $48 \times  24$ &  4  & 0.16667 & 0.9 & 2.9 & 110,318 \\
\midrule
 10 & $16 \times   8$ &  4  & 0.50000 & 0.9 & 2.1 & 1000 \\
    & $20 \times  10$ &  4  & 0.40000 & 0.9 & 2.1 & 1000 \\
    & $24 \times  12$ &  4  & 0.33333 & 1.0 & 2.5 & 1000,1000 \\
    & $32 \times  16$ &  4  & 0.25000 & 1.0 & 2.7 & 900,1000 \\
    & $48 \times  24$ &  4  & 0.16667 & 1.2 & 4.0 & 670,657 \\
\midrule
 20 & $16 \times   8$ &  4  & 0.50000 & 5.4 & 1.9 & 1000 \\
    & $20 \times  10$ &  4  & 0.40000 & 9.9 & 1.8 & 1000 \\
    & $24 \times  12$ &  4  & 0.33333 & 4.4 & 2.0 & 850 \\
    & $32 \times  16$ &  4  & 0.25000 & 7.4 & 2.3 & 850,1000 \\
    & $48 \times  24$ &  4  & 0.16667 & 7.4 & 3.5 & 301,677 \\
\midrule
 30 & $20 \times  10$ &  6  & 0.60000 & 1.3 & 2.9 & 950 \\
    & $24 \times  12$ &  6  & 0.50000 & 1.3 & 2.4 & 950 \\
    & $32 \times  16$ &  6  & 0.37500 & 1.7 & 2.3 & 975 \\
    & $48 \times  24$ &  6  & 0.25000 & 1.5 & 2.3 & 595,837 \\
    & $16 \times   8$ &  4  & 0.50000 & 1.4 & 1.9 & 1000 \\
    & $20 \times  10$ &  4  & 0.40000 & 1.2 & 2.7 & 950 \\
    & $24 \times  12$ &  4  & 0.33333 & 1.2 & 2.1 & 900 \\
    & $32 \times  16$ &  4  & 0.25000 & 1.3 & 1.8 & 900,1000 \\
    & $48 \times  24$ &  4  & 0.16667 & 1.3 & 4.3 & 150 \\
\midrule
 50 & $16 \times   8$ &  4  & 0.50000 & 1.1 & 1.8 & 1000 \\
    & $20 \times  10$ &  4  & 0.40000 & 1.2 & 1.8 & 1000 \\
    & $24 \times  12$ &  4  & 0.33333 & 0.8 & 2.0 & 1000 \\
    & $32 \times  16$ &  4  & 0.25000 & 1.3 & 2.0 & 900,1000 \\
    & $48 \times  24$ &  4  & 0.16667 & 1.3 & 2.2 & 467 \\
\midrule
100 & $16 \times   8$ &  4  & 0.50000 & 1.4 & 2.7 & 1000 \\
    & $20 \times  10$ &  4  & 0.40000 & 1.4 & 4.2 & 1000 \\
    & $24 \times  12$ &  4  & 0.33333 & 1.3 & 1.8 & 1000 \\
    & $32 \times  16$ &  4  & 0.25000 & 1.3 & 2.0 & 950,1000 \\
    & $48 \times  24$ &  4  & 0.16667 & 1.5 & 2.3 & 602 \\
\bottomrule
\end{tabular}

